Fast Gunrock Subgraph Matching (GSM) on GPUs

In this paper, we propose a GPU-efficient subgraph isomorphism algorithm using the Gunrock graph analytic framework, GSM (Gunrock Subgraph Matching), to compute graph matching on GPUs. In contrast to previous approaches on the CPU which are based on depth-first traversal, GSM is BFS-based: possible matches are explored simultaneously in a breadth-first strategy. The advantage of using BFS-based traversal is that we can leverage the massively parallel processing capabilities of the GPU. The disadvantage is the generation of more intermediate results. We propose several optimization techniques to cope with the problem. Our implementation follows a filtering-and-verification strategy. While most previous work on GPUs requires one-/two-step joining, we use one-step verification to decide the candidates in current frontier of nodes. Our implementation has a speedup up to 4x over previous GPU state-of-the-art implementation.

==> tex/acks.tex <==
Thanks to Seshadhri Comandur for providing the CPU baseline code for comparisons.
We appreciate the funding support of
DARPA XDATA under grants US Army award W911QX-12-C-0059, DARPA STTR awards D14PC00023 and
D15PC00010 as well as the National Science Foundation under grants CCF-1017399 and OCI-1032859, and a Lawrence Berkeley
Laboratory internship. Thanks also to NVIDIA for equipment
donations and server time.

